From Effectiveness to Efficiency: Uncovering Linguistic Bias in Large Language Model-based Code Generation

Large Language Models (LLMs) have demonstrated promising capabilities for code generation. While existing benchmarks evaluate the correctness and efficiency of LLM-generated code, the potential linguistic bias - where code quality varies based on the natural language used to describe programming tasks - remains underexplored. In this paper, we aim to investigate this linguistic bias through the lens of English and Chinese. To facilitate our investigation, we present a unified evaluation framework comprising a curated dataset of 52 Python programming questions with parallel bilingual task descriptions, automated correctness verification, and efficiency quantification tools based on runtime complexity estimation. Based on this framework, we conduct the first empirical study towards the linguistic bias in LLM-generated code on eight popular LCGMs, as well as GPT-3.5-Turbo and GPT-4. We observe that these LCGM-generated code show different correctness on an average of 12% bilingual programming tasks, where 39% also exhibits diverse efficiency. Our findings indicate that LLMs commonly exhibit linguistic bias for code generation.

==> src/bg.tex <==
\section{BACKGROUND}
\label{sec:bg}

% Firstly, we would like to provide a brief introduction to the basic knowledge of Large Code Generation Models (LCGMs). Furthermore, we will discuss the existing benchmarks for evaluating the code generation capabilities of LCGMs and their limitations, which motivates the necessity and significance of this study.

% \subsection{Large Code Generation Models}
% \label{sec:bg_lcgm}

% \todo{There is a purpose of why we write background. Here, we should introduce training corpus, so that it is obvious that these models are english heavy training and PLs are more similar to English, and hence, it is natural to wonder if the Chinese support is good. namely, we naturally tell them the motivation of why we need a study like this.}

% \todo{Reorganize this paragraph. Firstly, Bias about Code Model. Second, introduce linguistic bias, discuss the linguistic bias of LLM (corpora imbalance), and then use the following content to introduce an analysis and concern about why this problem may also be prevalent in Code Model.}

Large Language Models~(LLMs) denote language models characterized by billions of parameters, meticulously trained on extensive textual corpora to excel in various language processing assignments. 
% However, as a prototypical data-driven software, language models are likely to exhibit various defects due to the quality of training corpora~\cite{}. 
% Recent research has highlighted a concerning issue of language bias in large language models. 
% Due to the severe imbalance in training data across different languages, these models often exhibit significantly poorer performance on low-resource languages compared to high-resource languages, particularly English.
Particularly, Large Code Generation Models (LCGMs) undergo training and fine-tuning procedures specifically designed for programming languages, thereby augmenting their proficiency in executing software engineering tasks~\cite{sridhara2023chatgpt, mastropaolo2021studying}.
% The success of these models can be attributed to their training on vast corpora of code and natural language data, which allows them to learn the intricate patterns, syntax, and semantics of programming languages.
Testing and evaluating the quality of code generated by LCGMs from various perspectives is a crucial mission within the software engineering community. Numerous efforts have been dedicated to developing unified evaluation benchmarks to assess the functional correctness of LCGM-generated code~\cite{chen2021evaluating, austin2021program}, or exploring the robustness of AI Coders through techniques like metamorphic testing~\cite{li2023cctest,yang2024important}.


However, as a prototypical data-driven software, language models are likely to exhibit various defects due to the quality of training corpora. 
A typical issue is linguistic bias, which arises from the severe imbalance in the distribution of training corpora across languages, leading to models performing significantly better on high-resource languages such as English compared to low-resource languages~\cite{xu2024survey}.
Unfortunately, this issue may be just as or even worse with LCGMs.
The training corpora used for these LCGMs typically consist of a diverse collection of open-source code repositories, such as those hosted on GitHub~\cite{allamanis2018survey}. 
These repositories encompass a wide range of programming languages, \eg, Python, Java, C++, and JavaScript.
However, it is important to recognize that these repositories are English-heavy, \ie, project descriptions, functional documentations, code comments, and issue discussions are always written in English, as it is the predominant language used in global software development \cite{tomassetti2014empirical}. Additionally, many programming languages, such as Python and Java, have syntax and keywords that closely resemble English words and phrases \cite{pane2001studying}. 
Consequently, the datasets used for training LCGMs are heavily skewed towards English-language content.
This linguistic disparity raises concerns regarding the effectiveness of LCGMs in supporting and generating code for tasks presented in languages other than English, particularly those with distinct linguistic structures.
Naturally, this leads to an urgent need for an in-depth analysis of whether LCGMs exhibit consistent capabilities and quality in generating code across different languages.
% Unfortunately, existing code generation evaluation benchmarks (\eg, HumanEval~\cite{chen2021evaluating} and MBPP~\cite{austin2021program}) fail to address this question, as they predominantly focus on English programming challenges.
% Besides, these benchmarks focus on providing unit test cases to verify the correctness of code generated by LCGMs. In software engineering practice, assessing code quality often requires consideration of additional factors beyond correctness, such as code efficiency.





==> src/case_study.tex <==


\subsection{Case Study}
\label{sec:case_study}



\autoref{fig:motivation} illustrates a pair of practical examples for GPT-3.5-Turbo on bilingual programming tasks.
In the first example in~\autoref{fig:motivation}(a), GPT-3.5-Turbo generates the correct code for the Chinese input but fails to do so for the English input. 
Specifically, the solution ``return total//n'' (marked in red) does not align with the task description of returning the result "in a rounded integer." 
This further emphasizes the need for an interpretability-driven comprehensive study regarding which key entities or information from input problems are captured by LLMs for different input languages.

Moreover, we find that even when LLMs generate functionally correct code for both English and Chinese inputs, there can still be significant differences in the efficiency of the generated code.
As shown in the second example in~\autoref{fig:motivation}(b), the code generated for the Chinese input is less efficient than that for the English input. The average execution time complexity of the code generated for the Chinese input is $O(n^2)$ due to the presence of nested loops. In contrast, the code generated for the English input has an average time complexity of only $O(n \ast \log (n))$, thanks to the more concise and efficient library call of ``sort()''. 
This may inspire us that the subjective enthusiasm of LLMs for library API calls may affect the overall efficiency of their generated code.
It is worth noting that to better control variables and ensure that the Chinese-English differences in the input exist only in the programming question descriptions, we used the same English prompt for code generation in both languages.


% These examples, discovered through testing GPT-3.5-Turbo, underscore the need for a thorough and systematic evaluation of LLMs' performance on bilingual coding tasks. By identifying and quantifying differences in correctness, efficiency, and other relevant metrics across languages, we can gain valuable insights into the strengths and weaknesses of LLMs and work towards developing more robust and equitable code generation models.


% This discrepancy in performance across languages suggests potential biases or inconsistencies in the LLM's understanding and generation capabilities.
% Recent work by CodeApex~\cite{} has also revealed a similar issue, where LLMs achieve different Pass@K scores on bilingual university programming assignments across English and Chinese. 

==> src/design.tex <==
\section{Evaluation Framework}
\label{sec:design}

% In this section, we introduce our proposed framework for quantitatively measuring and evaluating the performance of CGM-generated code, thereby underpinning observations on bilingual performance disparities.

\begin{figure*}[!t]
    \centering
    % \sizebox{1.0}{
    \includegraphics[width=\linewidth]{figs/overview-2.pdf}
    % }
    \caption{The workflow of our evaluation.}

    \label{fig:overview}
    % \vspace{-10pt}
\end{figure*}





% \subsection{Goals and Research Questions}
% \todo{previously, you should have mentioned the motivation of doing this study. Here, you set the goals of this study, and in order to achieve the goal, we have a setup and a list of questions to answer. You should also put some discussions on the challenges as your design correspnods to  these challenges.}

% \update{
% To investigate whether LLMs perform consistently in code generation tasks across English and Chinese programming scenarios, we analyze the quality differences of the generated code in terms of correctness and efficiency. 

% To investigate the performance disparities of LLMs in generating code across English and other languages, we select Chinese as a comparative case study.
% Chinese is one of the most widely spoken language globally and also one of the most popular language among developers, including deverlopers and targeted users of LLMs.
% LLM has garnered substantial attention within the software engineering community due to the rapid expansion of the Chinese software industry~\cite{cyclesTopicSoftwareIndustry}.
% From the LLM aspect, most of them support Chines but may not other languages, due to the large Chinese corpus, e.g., documentation in Chinese on GitHub repositories.
% As such, most LLMs can perform well on leader boards using Chinese prompts.
% Moreover, Chinese exhibits significant linguistic divergence from English in terms of its writing system, grammatical structure, and lexical inventory \cite{mcenery2010corpus}, presenting a distinct challenge for LLMs predominantly trained on English-heavy corpora.
% Our study aims to conduct a fine-grained comparative analysis of the code generation quality(\ie, both correctness and efficiency) of existing LLMs when presented with programming tasks in English and Chinese. 
% }

% To investigate the linguistic bias via differential evaluating on quality disparities of LLM-generated code for input prompts in English and other languages, we select Chinese for a comparative case study. 
% Chinese is one of the most widely spoken languages globally and also one of the most popular languages among software developers and targeted users of LLMs. 
% Owing to the rapid growth of the Chinese software industry~\cite{cyclesTopicSoftwareIndustry}, the scale of Chinese corpora (\eg, GitHub repositories with Chinese documentation) is substantial, relative to other non-English languages.
% As such, most LLMs show strong performance on leaderboards related to Chinese programming tasks~\cite{fu2023codeapex}.
% LLMs have garnered substantial attention within the software engineering community due to the rapid expansion of the Chinese software industry~\cite{cyclesTopicSoftwareIndustry}.
% %%
% From the LLM perspective, most of them support Chinese but may not support other languages, due to the large Chinese corpus, such as documentation in Chinese on GitHub repositories. 
% As such, most LLMs can perform well on leaderboards using Chinese prompts.
%%
% Moreover, Chinese exhibits significant linguistic divergence from English in terms of its writing habit, grammatical structure, and lexical inventory~\cite{mcenery2010corpus}, presenting a distinct challenge for LLMs predominantly trained on English-heavy corpora.
%%
% Our study aims to conduct a fine-grained differential evaluation on the quality of LLM-generated code, encompassing both correctness and efficiency, when identical programming tasks are described in English and Chinese within the LLM input prompt.

% \update{
% However, this evaluation encounters several challenges.
% Firstly, there is a shortage of high-quality bilingual parallel programming question datasets. 
% The datasets used in current evaluation benchmarks are typically designed for individual natural languages.
% Secondly, while current benchmarks primarily focus on verifying the correctness of LLM-generated code, it is crucial, however efficiency is also a fundamental property that warrants significant attention, yet current benchmarks fall short in providing well-developed assessment tools.
% Thirdly, recent studies~\cite{liu2024your} have highlighted concerns regarding the sufficiency of current correctness validation benchmarks. Relying on a limited set of manually crafted unit test cases to verify code correctness may fall short of providing a satisfied coverage of the code functionality.
% To address these challenges, we propose a novel evaluation framework in this paper that includes a carefully curated bilingual parallel programming question dataset. 
% This framework enables us to validate the correctness of the generated code and estimate its execution performance under various inputs, thereby facilitating the assessment of the correctness and efficiency of LLM-generated code for bilingual programming questions and further exploring the quality differences.
% Ultimately, based on the proposed framework, we aim to answer the following research questions:
% % }

% Large code generation models (LLMs) always support multiple input languages, making a significant contribution to transforming the productivity experience of developers worldwide in different language environments. However, a key concern arises regarding the consistency of LLMs in generating high-quality code across different input languages. Can LLMs produce code of equally exceptional quality for identical programming tasks described in diverse languages? As a preliminary exploration, we aim to investigate the variations in code quality generated by LLMs in bilingual programming questions, considering the active developer communities using English and Chinese as widely used languages.

% In the realm of software engineering, correctness and efficiency stand as fundamental attributes for evaluating program or code quality. 
% correctness ensures that the code output aligns with expected results, while efficiency focuses on code execution performance, including its ability to provide timely responses within predefined limits and maintain acceptable time consumption as input size increases.

% In this work, we aim to answer the following research questions:

% \begin{itemize}
%     \item RQ1: Is the code generated by LLMs equally correct when programming questions are presented in either English or Chinese?
%     \item RQ2: Is the code generated by LLMs equally efficient when programming questions are presented in either English or Chinese?
%     \item RQ3: What is the impact of prompting methods on LLM's linguistic bias?
% \end{itemize}
% \todo{update}

% By addressing these research questions, we aim to provide insights into the capabilities and limitations of LLMs in generating code for bilingual programming questions, as well as the role of prompting in enhancing their performance. Our findings can contribute to the development of more effective and efficient code generation models that can handle diverse language inputs.

% \subsection{Evaluation Framework}

In this paper, we choose English and Chinese as the two languages for our evaluation based on three key considerations. 
First, English serves as the dominant programming language globally, while Chinese also represents one of the most widely spoken languages in the world. This combination effectively represents the linguistic environment of a significant portion of developers worldwide. Moreover, if substantial linguistic bias exists between these two commonly used languages, it suggests that the issue may be even more pronounced in low-resource languages. 
Second, English and Chinese exhibit fundamental differences in grammatical structure and vocabulary~\cite{mcenery2010corpus}, providing an ideal test bed for examining how LLMs handle code generation across linguistically diverse inputs. 
Finally and crucially, it is limited by our expertise in linguistic, ensuring accurate understanding and quality control of prompts—a critical factor in maintaining the validity of our evaluation.


\subsection{Design Overview}

To enable simultaneous measurement of the correctness and efficiency of LLM-generated code, we propose a framework, consisting of four steps: dataset collection, code generation, correctness verification, and performance estimation.
\autoref{fig:overview} illustrates our framework.
We begin by selecting appropriate programming questions and canonical solutions from mainstream LLMs benchmarks, and meticulously preparing bilingual (English-Chinese) versions. 
We also construct an test input generator to automatically create test inputs of various sizes for each question (\WC{1}).
Next, we input the bilingual programming questions into the LLM separately, to obtain the generated code (\WC{2}). 
% This allows us to investigate the impact of prompting on the quality of generated code in both languages.
To assess the correctness, we verify the correctness of the generated code by comparing its output results with the canonical solution, i.e., conducting comprehensive unit testing under a large number of inputs generated by the test input generator. (\WC{3}). 
% This quantitatively measures the ability of LLMs to produce functionally correct code for bilingual programming questions.
To evaluate the efficiency, we collect ``input size-execution time'' pairs for functionally correct code by running them with different input sizes and fitting them to common time complexity expressions to estimate the average execution performance (\WC{4}).
% This helps us assess the efficiency and identify potential performance differences between the English and Chinese versions of the same question.
Besides, this framework also supports the investigation of the impact of prompting by allowing customizing various prompts used by code generation.
With the verified correctness and average execution performance, we gain insights into the quality of LLM-generated code.
% Our framework comprehensively investigates the correctness, efficiency, and impact of prompting on LLMs' ability to handle bilingual programming questions (RQ1, RQ2, and RQ3), contributing to the development of advanced, language-agnostic code generation models.

% \begin{figure*}[t!]
%     \centering
%     % \sizebox{1.0}{
%     \includegraphics[width=0.9\linewidth]{figs/testexamples.pdf}
%     % }
%     \caption{An example in our test suite.}

%     \label{fig:examples}
%     % \vspace{-10pt}
% \end{figure*}



\subsection{Dataset Collection}

Existing benchmarks usually provide many meticulously crafted programming tasks for evaluating the correctness of LLM-generated code, which typically include task descriptions, program entries, input/output examples, canonical solutions, and a few unit test cases. 
We use three popular datasets, HumanEval~\cite{chen2021evaluating}, MBPP~\cite{austin2021program}, and LeetCode~\cite{leetcode} as the initial question list, where requiring LLMs to fill in Python code segments based on specific task descriptions and program entry points.
To keep the quality and suitability of the test suite, we then filter programming questions based on the following criteria: (i) ensuring that the tasks are of moderate difficulty level to prevent LLMs from struggling to generate correct answers in both bilingual inputs, (ii) ensuring that the tasks have multiple potential solutions to increase the likelihood of observing performance differences, and (iii)
ensuring that the tasks take a variable with varying dimensionality as inputs, \eg, an array or list, where the execution time of the solutions is strongly correlated with the dimensionality of the input variable.
In order to identify candidate questions that satisfy criterion (ii), we search these questions on the Internet, and since the questions are from publicly available datasets, it is easy to find some reference solutions for them. We make sure that at least two solutions with different time complexity exist for the selected problems.
Specifically, two authors in the fields of software engineering independently conduct the data collection. 
The intersection of these two sets passed to a third author with extensive programming competition experience for a double check.
After careful collection and filtration, we ultimately select 52 programming questions, covering a diverse range of problem types, such as dynamic programming, string processing, array enumeration, and more. 
Although this dataset is only half the size of HumanEval, it is sufficient to show the quality differences in LLM-generated code for bilingual inputs, as demonstrated in \autoref{sec:eval}.


The questions collected from HumanEval and MBPP are initially in English. 
Two authors proficient in both languages meticulously translate them into Chinese. 
For questions from LeetCode, which provides official bilingual versions, we adopt them directly. 
We thoroughly check all bilingual question pairs to ensure their consistency in task descriptions and adherence to the respective language conventions.
Additionally, for each programming question, we design an automated test input generator, denoted as \(G\). 
It takes an input size parameter $n$ that determines the dimensionality of the generated variables. These variables are tailored to act as unit test inputs for the specific programming questions.
By varying the size parameter, $G$ can generate a wide range of inputs, from small and simple cases to large and complicated ones. 
By intentionally incorporating randomness into the input generation process, we aim to create a diverse set of test cases to thoroughly validate the correctness of LLM-generated code and to better characterize its average efficiency when faced with a large number of test inputs.

Our test suite can be formally represented as $\mathcal{D} = \langle Q, S, G \rangle$, where $Q$ is the programming question, $S$ is the canonical solution, and $G$ is the test input generator. 
$Q$ consists of a task description, an entry point function name, and reference input/output. 
For each question \(q \in Q\), we have two bilingual parallel versions, \(q_{en}\) and \(q_{zh}\), presented in English and Chinese, respectively.
$S$ is the canonical solution of the given programming questions, which is used to produce ground truth outputs for correctness verification.
$G$ is a crucial component, serving as the input generator. 
By leveraging $G$, we can automatically generate a diverse set of test cases, saving time and effort compared to manually generating inputs while maintaining high quality and coverage.


\subsection{Code Generation}

While LLMs demonstrate impressive code generation capabilities, accurately extracting the desired code from their responses remains an engineering challenge.
Typically, many LLMs struggle to precisely terminate their generation process after completing the target function, often continuing to generate extraneous code until reaching the maximum token limit~\cite{guo2024stop}. 
Directly executing such code in a sandbox environment, e.g., provided by HumanEval, frequently triggers parsing errors or interference from the additional functions.
To minimize this interference, we perform an Abstract Syntax Tree (AST) based analysis on the generated results. 
By traversing the AST, we identify and extract only the code segments corresponding to the target function specified by the entry point. 
This targeted extraction ensures that only the code essential to the function's execution is retained, thereby reducing the likelihood of errors that may arise from the inclusion of non-essential or erroneous code segments. 
This preprocessing is crucial in accurately assessing the correctness of the LLMs' outputs and ensuring that the evaluation is not compromised by the LLMs' tendency to generate superfluous code.

% \todo{there are also some engineering challenges, e.g., extracting the answers from the responses. if you solved them, you should discuss them.}

\subsection{Correctness Verification}

As discussed earlier, only a few test cases in existing benchmarks are often insufficient to guarantee thorough functionality correctness judgement, such a concern is also highlighted in recent studies~\cite{liu2024your}.
To ensure the adequacy of unit testing, we automatically generate larger-size test cases for correctness verification.
As aforementioned, our collected dataset includes an input generator, which can generate random inputs of a specified size. 
With the canonical solution \(S\), we can automatically synthesize reference outputs, i.e., ground truth. 
Therefore, we can conduct more comprehensive unit testing.
We draw inspiration from HumanEval's approach, which involves executing the code in a sandbox environment and verifying correctness by comparing the output of the LLM-generated code with the synthesized ground truth.
By comparing the differences in functionality correctness of LLM-generated code across bilingual versions of the same programming question, we can conduct further statistical analysis to support the investigation of RQ1.
Furthermore, we filter out the functionally correct code based on extensive unit testing. 
Prioritizing correctness verification lays a solid foundation for subsequent performance estimation, as discussing the performance merits of code with inherent functional errors lacks practical significance. 
% By focusing on the functionally correct code, we can provide meaningful insights into the correctness of LLMs in generating accurate solutions to bilingual programming questions.

% Existing benchmarks often include a small number of handwritten unit test cases to test code functionality. However, we have found that these unit test cases are often insufficient to guarantee thorough testing, a concern also highlighted in recent studies~\cite{}. 
% To ensure the adequacy of unit testing, we need to conduct tests on a larger size. As mentioned earlier, our collected dataset includes an input generator, which can generate random inputs of specified size. With the canonical solution \(S\), we can generate reference outputs, i.e., ground truth. Therefore, we can conduct more comprehensive unit testing.
% We draw inspiration from HumanEval's approach, which involves executing the generated code in a sandbox environment and verifying correctness by comparing the output of the generated code $C_{en}, C_{zh}$ with the canonical solution \(S\). 
% Ultimately, we filter out the functionally correct code.
% Prioritizing correctness validation lays a solid foundation for subsequent performance estimation. We suppose that discussing the performance merits of code with inherent functional errors lacks practical significance. 


\subsection{Performance Estimation}

% \begin{table}[]
%     \centering
%     \small
%     \caption{Common time complexity types.}
%     \begin{tabular}{cc}
%     \hline
%     Type         &  Expression  \\ \hline
%     Constant     &  $time = a (sec)$      \\
%     Logarithmic  & $time = a*log(n) + b (sec)$     \\
%     Linear       & $time = a*log(n) + b (sec)$      \\
%     Linearithmic & $time = a*n*log(n) + b (sec)$     \\
%     Quadratic    & $time = a*n^2 + b (sec)$       \\
%     Cubic        & $time = a*n^3 + b (sec)$       \\
%     Exponential  &  $time = a^n + b (sec)$\\ \hline
%     \end{tabular}
%     \label{tab:bigO}
% \end{table}

\begin{table}
    \centering
    \small
    \caption{Common time complexity types.}
    \begin{tabular}{cc}
    \hline
    Type         &  Expression  \\ \hline
    Constant     &  $time = a \, \text{(sec)}$      \\
    Logarithmic  & $time = a \log(n) + b \, \text{(sec)}$     \\
    Linear       & $time = a n + b \, \text{(sec)}$      \\
    Linearithmic & $time = a n \log(n) + b \, \text{(sec)}$     \\
    Quadratic    & $time = a n^2 + b \, \text{(sec)}$       \\
    Cubic        & $time = a n^3 + b \, \text{(sec)}$       \\
    Exponential  &  $time = a^n + b \, \text{(sec)}$\\ \hline
    \end{tabular}
    \label{tab:bigO}
\end{table}


Accurately characterizing and evaluating the execution performance or time complexity of arbitrary code is often challenging, especially when the LLM-generated code may contain external function calls.
In our framework, we estimate the execution performance by sampling a large number of inputs and observing the changes in the execution time of the LLM-generated code as the input size grows. 
Recall that with the input generator \(G\), we can sample test inputs of various sizes for the under-measuring code by generating input variables with different dimensions, thereby enabling us to profile actual execution time for LLM-generate code across different input sizes.


Initially, when constructing the input generator, we empirically set an initial maximum input size $N_{max}$ for each programming question, taking into account the complexity of the canonical solution.
This value is set to be sufficiently large, allowing us to divide it into many segments to sample different input sizes.
However, a problem arises as the LLM-generate code could have a higher complexity than the canonical solution, leading to excessively long execution times and making the overall evaluation time prohibitively expensive. 
To address this problem, we design an adaptive mechanism for adjusting the maximum input size. 
Following HumanEval, we first set a maximum time limit $T_{max}$ for code execution.
Subsequently, we examine the execution of each LLM-generated code to determine if it triggers a timeout when processing inputs of size $N_{max}$. In the event of a timeout, we iteratively decrease $N_{max}$ by half until the execution satisfies the $T_{max}$ constraint.

% To determine the maximum sampling size, we need to balance two factors: (i) if the size is too small, the execution time may be significantly affected by other factors such as thread switching; (ii) if the size is too large, the experiments will be overly time-consuming.
% Considering these two points, we adaptively change the maximum sampling size.
% First, we set an upper limit $T_{max}$ for the code execution time, namely, the acceptable longest execution time. 
% Then, by gradually increasing the input size and observing the actual execution time, we can find the maximum input size $N_{max}$ that satisfies the $T_{max}$ constraint. 



With the maximum input size $N_{max}$, we divide it into $seg$ equal parts and obtain an increasing sequence of input sizes:
$$N = {n_i | n_i = i \cdot \frac{N_{max}}{seg}, i = 1, 2, \dots, seg}$$
% \todo{This paragraph is not very clear. most importantly, what is the input size? input size is the value range of an analog conversion input that is converted to engineering units. Are you sure we use input size here? Or if you use it, at least you define it, I am not sure if this is the standard term. For us, it is more of the input dimensions?}

For each input size $n_i$, we perform $k$ samplings, record the execution time of each run, and take the average as the execution time estimate $t_i$ under that input size. This way, we obtain a set of ``input size-execution time'' pairs:
$$NT = {(n_i, t_i) | n_i \in N, t_i = \frac{1}{k}\sum_{j=1}^{k}t_{ij}, i = 1, 2, \dots, seg}$$
where $t_{ij}$ represents the execution time of the $j$-th sampling when the input size is $n_i$.



We present a summary of seven prevalent time complexity types, as illustrated in \autoref{tab:bigO}. 
To determine the most matching time complexity type and corresponding mathematical expression, we employ the least squares method to perform a regression analysis~\cite{draper1998applied} on the time series data $(NT)$. 
This approach enables us to identify the closest matching complexity type.
Additionally, we assign a score ranging from 1 to 7 to each time complexity type, following the order presented in \autoref{tab:bigO}. 
Lower scores indicate higher efficiency in terms of actual code execution. With this scoring mechanism, we can quantitatively compare the efficiency of two code pieces in actual sampling-based execution.

\input{src/tf/tab_metric.tex}
\subsection{Measurement Metrics}\label{sec:metrics}



To systematically evaluate the discrepancies in code generation capabilities of LLMs when handling bilingual versions of identical programming problems, we comprises seven carefully designed metrics: four metrics quantify the differences in code correctness across languages, while three metrics measure the variations in code execution efficiency (see \autoref{tab:metricssummary}). For detailed definitions and analytical methodologies of these metrics, please refer to ~\autoref{sec:appendix_metrics}.

% Regarding the efficiency differences in the generated code, there is no ground truth like in the case of correctness. Based on the estimated complexity expressions, we can compare any pair of generated code in the bilingual setting, to determine whether they exhibit the same performance level or if one outperforms the other. Furthermore, we evaluate the following metrics on the subset of problems for which the LLMs can generate correct code in both languages:
% $Perf_{en}$, represent the proportion of problems where the performance of $C_{en}$ is better than $C_{zh}$.
% $Perf_{zh}$, represent the proportion of problems where the performance of $C_{zh}$ is better than $C_{en}$.
% The sum of these two metrics, denoted as $DiffP$, represents the proportion of problems for which the LLMs can generate correct code in both languages but with significantly different performance levels.

% Formally, let $D_{bi}$ be the subset of problems in the test suite $D$ for which the LLM can generate correct code in both English and Chinese. Then, $Perf_{en}$, $Perf_{zh}$, and $DiffP$ can be defined as follows:

% \begin{equation}
% Perf_{en} = \frac{|{Q \in D_{bi}: C_{en} \text{ performs better than } C_{zh}}|}{|D_{bi}|}
% \end{equation}

% \begin{equation}
% Perf_{zh} = \frac{|{Q \in D_{bi}: C_{zh} \text{ performs better than } C_{en}}|}{|D_{bi}|}
% \end{equation}

% \begin{equation}
% DiffP = Perf_{en} + Perf_{zh}
% \end{equation}

% By evaluating these metrics, we can gain insights into the performance differences between the English and Chinese code generated by the LLMs, specifically focusing on the problems where the LLMs can generate correct code in both languages. A higher value of $DiffP$ indicates that the LLMs exhibit more significant performance disparities between the two languages, even when they can generate functionally correct code for the same problem.

\subsection{Target LLMs}

In our study, we evaluated a diverse set of LLMs, including both open-source and commercial solutions. 
Our model selection prioritizes three key criteria: multilingual capabilities (English/Chinese), architectural diversity to capture linguistic bias generalizability, and computational feasibility (i.e., the model has most 34B parameters).
We selected five families of open-source LLMs: CodeGen2.5-7B~\cite{Nijkamp2023codegen2}, StarCoder-13B~\cite{li2023starcoder}, CodeGeeX-6.7B~\cite{zheng2023codegeex}, CodeLlama (7B/13B/34B)\cite{roziere2023CodeLlama}, and DeepSeek-Coder (7B/33B)\cite{guo2024deepseek}. Additionally, we included two commercial close-source models, GPT-3.5-Turbo and GPT-4~\cite{gpt3.5-oepnai}, resulting in a total of ten evaluated models. 
% For certain in-depth analyses, we focused on the smaller versions (≤7B parameters) of the open-source models due to computational constraints.
More details on the selected models can be found in \autoref{sec:appendix_models}.


% \subsection{Parameter Configuration}

% In our experiments, the maximum time limit $T_{max}$ is 6 seconds, the number of sampling $k$ is 100, and the number of segments $seg$ is 50.
% Another important parameter when utilizing LLMs is the temperature ($t$), which typically ranges from 0 to 1. 
% Lower temperature values result in more deterministic and concentrated outputs, while higher values lead to more diverse and exploratory generations. 
% We select two common temperature values, 0.2 and 0.8, to better observe the impact of this parameter on the quality of the generated code~\cite{OpenAI-API-doc}.


==> src/discussions.tex <==
\section{Discussions}
\label{sec:discussions}

\subsection{Discussions and Suggections}


\noindent\textbf{Thinking more deeply about linguistic bias.} Our study results indicate that, in most cases, LCGMs indeed tend to generate higher-quality code for English inputs. Here, we discuss a possible reason for this phenomenon. As recent research has shown, English functions as the ``native language'' of LLMs, implying that their internal state space appears to be accustomed to translating other languages into English before formulating responses~\cite{wendler2024llamas}. 
This translation process may lead to a degradation in prompt quality and a loss of information.


\noindent\textbf{Comprehensive Multilingual Code Generation Quality Assessment.} Based on the results from RQ1 and RQ2, our study has revealed significant disparities in the effectiveness and efficiency of LCGMs in generating code for bilingual~(Chinese and English) programming. It is reasonable to infer that such differences are not confined to these two languages but may represent a broader phenomenon. 
Emerging research has increasingly investigated the multilingual understanding and generation capabilities of Large Language Models~\cite{zhang2024m3exam}, and similar scrutiny must be directed towards LCGMs.
Moreover, effectiveness and efficiency are only two aspects of code quality, other important attributes such as security, readability, and maintainability also deserve consideration. Therefore, expanding the scope of quality assessment to include these additional attributes is a valuable direction for future research.

\noindent\textbf{Developing Better Prompting Methods.} 
According to RQ3, the impact of different prompting strategies on the quality of LCGM-generated code is substantial. 
Prompting techniques are pivotal in the era of LLMs, and well-crafted prompts can significantly enhance the quality of generation~\cite{liu2023pre}. 
Investigating how to construct superior prompts that enable LCGMs to consistently produce high-quality code across different languages is of paramount importance.

% \noindent\textbf{Adaptive Temperature Tuning.} It has been observed that as the temperature parameter increases, LCGMs exhibit varying performance across languages, \ie, most LCGMs tend to prefer generating code of higher quality in English. Identifying the optimal temperature settings that allow LCGMs to perform best for each language could be a key factor in improving multilingual code generation.

In summary, one important message from this study is that the software engineering community should establish benchmarks and frameworks for evaluating the multilingual code generation capabilities of LCGMs, considering different code quality assessment metrics, input languages, prompting methods, and more. As an initial step, we have released our framework~\cite{ourrepo} and strongly encourage our readers to contribute more datasets and code quality measurements.


% albeit meticulously curated, 
\subsection{Threats to Validity}
\noindent
\textbf{Limited Dataset:} The dataset utilized in this study, despite careful designing, is limited to 52 bilingual programming questions, which may not sufficiently cover the diverse range of tasks LCGMs encounter in practical applications. Furthermore, the dataset only includes English and Chinese, potentially failing to capture the performance variations of LCGMs across a wider array of languages. This limitation stems from the requirement of strong language proficiency to ensure the quality of multilingual parallel data.

\noindent
\textbf{Limited LCGMs:} 
LCGMs are rapidly proliferating in number, and since our evaluation is based on the actual execution of a large amount of code generated by LCGMs, it is impractical to exhaustively cover all LCGMs.
We have made every effort to evaluate 10 popular models from 5 different open-source families and one leading commercial company.
However, the selected LCGMs serve as the foundation for many advanced LCGMs. Our evaluation method is universal and extendable to a broader range of models.

\noindent
\textbf{Evaluation Metrics:} The metrics employed in this study primarily focus on code correctness and efficiency, potentially neglecting other crucial aspects of code quality, such as readability, maintainability, and adherence to coding standards. The absence of these factors in the evaluation process may restrict the comprehensive understanding of the LCGM's performance.

To mitigate the threats and foster further research, we make our collected dataset and evaluation framework publicly available~\cite{ourrepo}. This initiative aims to empower researchers to expand the study by incorporating diverse programming tasks, languages, and quality assessment metrics, as well as to include a broader range of LCGMs in the comparison.

% By encouraging the community to conduct more comprehensive experiments across a wider range of LCGMs, we seek to contribute to a more robust and nuanced understanding of these models' capabilities and limitations in a multilingual coding context. This collaborative approach will not only help mitigate the identified threats to validity but also foster a more inclusive and comprehensive analysis of LCGMs' potential in the field of code generation.

==> src/motivation.tex <==
\section{MOTIVATION}
\label{sec:moti}



Contemporary LCGMs typically support a wide range of input languages, revolutionizing productivity tools for developers worldwide across diverse language environments. With English and Chinese being the most commonly used languages and the primary communities in software engineering~\cite{}, an intriguing and noteworthy question arises: \textit{Can a LCGM produce consistent or equivalently quality codes for the same programming task descriptions expressed in English and Chinese respectively?}, which concerns the whether different developers can fairly experience the dividends of new LCGM technologies.

From a software engineering perspective, effectiveness and efficiency are two key attributes for evaluating program/code quality. The former refers to the functionality correctness of the code, while the latter concerns the execution performance of the code. 
Through our observations, we have noted significant differences in both the correctness and execution performance of code generated by LCGMs under bilingual input.
\autoref{fig:motivation} illustrates a pair of practical example.
In the first example, the LCGM generates a correct code for the Chinese input, but fails to do so for the English input, \ie, the solution ``return total//n'' is not in line with the task description of ``in a rounded integer''.
Recent work by CodeApex~\cite{} has also revealed a similar problem that LCGMs achieve different Pass@K scores on bilingual university programming assignments across English and Chinese. 
Furthermore, we find that even if LCGMs generate functionally correct code under bilingual inputs, there are still differences in their efficiency.
As shown in the second example, the code generated for the Chinese input is less efficient than that for the English input, \ie, the average execution time complexity of the code generated for the Chinese input is $O (n^2)$ due to the presence of nested loops. In contrast, for the Chinese input, is only $O (nlogn)$, due to the more concise and efficient library call of ``sort()''.


Existing LCGM evaluation benchmarks primarily gather a set of English programming problems and validate the functionality correctness of the code by providing a few manual unit test cases. 
This presents us with three challenges to the bilingual evaluation of LCGMs: \ding{172} the
absence of high-quality bilingual programming problem datasets; \ding{173} inadequate unit test cases to ensure thorough correctness verification; \ding{174} limited support/concern for measuring and comparing
the performance of generated codes.
These requirements and challenges motivate us to propose a framework for bilingual code quality assessment, aimed at capturing the effectiveness and efficiency of code generated by LCGMs across a range of bilingual programming problems. 
This framework enables us to further analyze the disparities in bilingual programming capabilities.







==> src/rq-para.tex <==
\subsection{About Configurable Parameters}
\label{sec:rq-para}

Our evaluation framework incorporates several configurable parameters. The calibration of these parameters is crucial, as excessively low values may introduce undue randomness, while overly high values can significantly increase computational time. To address this trade-off, we have meticulously adjusted these parameters.
To alleviate concerns regarding the reliability of our evaluation with respect to parameter selection, we conducted convergence experiments. These experiments aimed to verify the stability of our results across different parameter configurations. 
We randomly select 30 code snippets generated for different programming questions. We try maximum time limits \(T_{max}=6,8,10\), the number of samples \(k=100,150,200\), and the number of segments \(seg=50,100,200\). 
That means we increase the parameters used in the paper to observe the consistency of complexity estimation results. The results show that all 30 outcomes are consistent as Tmax changes, and 29 outcomes are consistent with changes in \(k\) and \(seg\). The only inconsistency arises from slight errors in quadratic fitting. 
Overall, our chosen parameter settings exhibit a strong stability in the assessment of results. The significant consistency observed across different parameter configurations enhances the reliability of our evaluation framework and supports the validity of our conclusions.





==> src/tf/correctness.tex <==

% \begin{table}[hbt]
% \begin{table}[]
%     \centering
%     \caption{Effectiveness Measurement Results.}
%     \tabcolsep=1.5pt
%     \begin{tabular}{|l|llll|llll|}
%     \hline
%                            & \multicolumn{4}{c|}{t = 0.2}                                                                          & \multicolumn{4}{c|}{t = 0.8}                                                                          \\
%     \multirow{-2}{*}{LCGM} & $CR_{en}$                    & $CR_{zh}$                    & $CR_{bi}$ & $CDR$                       & $CR_{en}$                    & $CR_{zh}$                    & $CR_{bi}$ & $CDR$                       \\ \hline
%     CodeGeeX               & \cellcolor[HTML]{E2EFDA}0.60 & 0.54                         & 0.54      & 0.06 & 0.62                         & \cellcolor[HTML]{FCE4D6}0.63 & 0.58      & \bf 0.10                        \\
%     CodeGen2.5             & 0.52                         & 0.52                         & 0.46      & \bf 0.12                        & 0.46                         & \cellcolor[HTML]{FCE4D6}0.48 & 0.40      & \bf 0.13                        \\
%     CodeLlama              & 0.50                         & \cellcolor[HTML]{FCE4D6}0.54 & 0.46      & \bf 0.12                        & \cellcolor[HTML]{E2EFDA}0.52 & 0.50                         & 0.46      & \bf 0.10                        \\
%     DeepSeek-Coder         & \cellcolor[HTML]{E2EFDA}0.63 & 0.58                         & 0.54      & \bf 0.13                        & \cellcolor[HTML]{E2EFDA}0.71 & 0.65                         & 0.63      & \bf 0.10                        \\
%     StarCoder              & 0.48                         & \cellcolor[HTML]{FCE4D6}0.52 & 0.44      & \bf 0.12                        & \cellcolor[HTML]{E2EFDA}0.58 & 0.56                         & 0.52      & \bf 0.10                        \\
%     GPT-3.5-Turbo          & 0.58                         & \cellcolor[HTML]{FCE4D6}0.64 & 0.58      & 0.08 & \cellcolor[HTML]{E2EFDA}0.7  & 0.66                         & 0.67      & 0.04 \\ \hline
%     Average                & 0.55                         & \cellcolor[HTML]{FCE4D6}0.56 & 0.50      &\bf  0.11                        & \cellcolor[HTML]{E2EFDA}0.60 & 0.58                         & 0.54      & \bf 0.10                        \\ \hline
%     \end{tabular}
%     \label{tab:rq1}
%     \vspace{-10pt}
    % \end{table}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table*}[tbp]
    \centering
    \caption{Results of Measurement on Correctness Difference.}
    
    \small
    \begin{tabular}{cccccccccc}
    \hline
     &  & \multicolumn{4}{c}{\(t=0.2\)} & \multicolumn{4}{c}{\(t=0.8\)} \\ \cmidrule(lr){3-6} \cmidrule(lr){7-10} 
    %  & \multirow{-2}{*}{Model} & CR\_en & CR\_zh & CR\_bi & CDR & CR\_en & CR\_zh & CR\_bi & CDR \\ \hline
    & \multirow{-2}{*}{LCGM} & $CR_{en}$                    & $CR_{zh}$                    & $CR_{bi}$ & $CDR$                       & $CR_{en}$                    & $CR_{zh}$                    & $CR_{bi}$ & $CDR$ \\ \hline
     & CodeGeeX(6.7B) & \cellcolor[HTML]{D9EAD3}0.60 & 0.54 & 0.54 & 0.06 & 0.62 & \cellcolor[HTML]{FCE5CD}0.63 & 0.58 & 0.14 \\
     & CodeGen2.5(7B) & 0.52 & 0.52 & 0.46 & 0.12 & 0.46 & \cellcolor[HTML]{FCE5CD}0.48 & 0.40 & 0.25 \\
     & CodeLlama(7B) & 0.50 & \cellcolor[HTML]{FCE5CD}0.54 & 0.46 & 0.12 & \cellcolor[HTML]{D9EAD3}0.52 & 0.50 & 0.46 & 0.17 \\
     & DeepSeek-Coder(13B) & \cellcolor[HTML]{D9EAD3}0.63 & 0.58 & 0.54 & 0.13 & \cellcolor[HTML]{D9EAD3}0.71 & 0.65 & 0.63 & 0.13 \\
     & StarCoder(13B) & 0.48 & \cellcolor[HTML]{FCE5CD}0.52 & 0.44 & 0.12 & \cellcolor[HTML]{D9EAD3}0.58 & 0.56 & 0.52 & 0.16 \\
     & CodeLlama(13B) & 0.46 & \cellcolor[HTML]{FCE5CD}0.56 & 0.44 & 0.13 & 0.54 & \cellcolor[HTML]{FCE5CD}0.58 & 0.50 & 0.12 \\
     & DeepSeek-Coder(33B) & 0.60 & \cellcolor[HTML]{FCE5CD}0.62 & 0.54 & 0.13 & \cellcolor[HTML]{D9EAD3}0.60 & 0.58 & 0.54 & 0.10 \\
    \multirow{-8}{*}{} & CodeLlama(34B) & 0.54 & \cellcolor[HTML]{FCE5CD}0.60 & 0.48 & 0.17 & \cellcolor[HTML]{D9EAD3}0.67 & 0.56 & 0.54 & 0.15 \\ \hline
     & GPT-3.5-Turbo & 0.58 & \cellcolor[HTML]{FCE5CD}0.64 & 0.58 & 0.08 & \cellcolor[HTML]{D9EAD3}0.70 & 0.66 & 0.67 & 0.05 \\
    \multirow{-2}{*}{} & GPT-4 & \cellcolor[HTML]{D9EAD3}0.65 & 0.63 & 0.61 & 0.06 & \cellcolor[HTML]{D9EAD3}0.71 & 0.65 & 0.65 & 0.06 \\ \hline
    \multicolumn{1}{l}{} & Average & 0.56 & \cellcolor[HTML]{FCE5CD}0.58 & 0.51 & 0.11 & \cellcolor[HTML]{D9EAD3}0.61 & 0.59 & 0.55 & 0.13 \\ \hline
    \end{tabular}
    \label{tab:rq1}
\end{table*}

==> src/tf/efficiency.tex <==
% \begin{table}[]
%     \centering
%     \caption{Efficiency Measurement Results.}
%     \setlength{\tabcolsep}{2pt}
%     \begin{tabular}{|l|ccc|ccc|}
%         \hline
%                                & \multicolumn{3}{c|}{t = 0.2}                                                                     & \multicolumn{3}{c|}{t = 0.8}                                                                     \\
%         \multirow{-2}{*}{LCGM} & \multicolumn{1}{l}{$PAR_{en}$} & \multicolumn{1}{l}{$PAR_{zh}$} & \multicolumn{1}{l|}{$PDR$} & \multicolumn{1}{l}{$PAR_{en}$} & \multicolumn{1}{l}{$PAR_{zh}$} & \multicolumn{1}{l|}{$PDR$} \\ \hline
%         CodeGeeX               & 0.17                            & 0.17                            & 0.34                         & \cellcolor[HTML]{E2EFDA}0.34    & 0.2                             & 0.54                         \\
%         CodeGen2.5              & 0.2                             & \cellcolor[HTML]{FCE4D6}0.23    & 0.43                         & 0.11                            & \cellcolor[HTML]{FCE4D6}0.25    & 0.36                         \\
%         CodeLlama              & 0.13                            & \cellcolor[HTML]{FCE4D6}0.27    & 0.4                          & \cellcolor[HTML]{E2EFDA}0.21    & 0.14                            & 0.34                         \\
%         DeepSeek-Coder          & 0.2                             & \cellcolor[HTML]{FCE4D6}0.23    & 0.43                         & \cellcolor[HTML]{E2EFDA}0.24    & 0.11                            & 0.34                         \\
%         StarCoder              & 0.17                            & \cellcolor[HTML]{FCE4D6}0.24    & 0.41                         & \cellcolor[HTML]{E2EFDA}0.26    & 0.13                            & 0.39                         \\
%         GPT-3.5-Turbo           & 0.06                            & \cellcolor[HTML]{FCE4D6}0.29    & 0.35                         & \cellcolor[HTML]{E2EFDA}0.22    & 0.19                            & 0.41                         \\ \hline
%         Average                & 0.16                            & \cellcolor[HTML]{FCE4D6}0.24                            & 0.39                         & \cellcolor[HTML]{E2EFDA}0.23                            & 0.17                            & 0.40                         \\ \hline
%         \end{tabular}
%     \label{tab:rq2}
%     \vspace{-10pt}
% \end{table}

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
\begin{table*}[tbp]
    \centering
    \caption{Results of Measurement on Efficiency Difference.}
    \small
    \begin{tabular}{cccccccc}
    \hline
    \multicolumn{2}{c}{} & \multicolumn{3}{c}{\(t=0.2\)} & \multicolumn{3}{c}{\(t=0.8\)} \\ \cmidrule(lr){3-5} \cmidrule(lr){6-8} 
    \multicolumn{2}{c}{\multirow{-2}{*}{LCGM}} & \multicolumn{1}{l}{$PAR_{en}$} & \multicolumn{1}{l}{$PAR_{zh}$} & \multicolumn{1}{l}{$PDR$} & \multicolumn{1}{l}{$PAR_{en}$} & \multicolumn{1}{l}{$PAR_{zh}$} & \multicolumn{1}{l}{$PDR$} \\ \hline
    & CodeGeeX(6.7B) & 0.17 & 0.17 & 0.33 & \cellcolor[HTML]{D9EAD3}0.34 & 0.20 & \cellcolor[HTML]{FFFFFF}0.54 \\
    & CodeGen2.5(7B) & 0.20 & \cellcolor[HTML]{FCE5CD}0.23 & 0.43 & 0.11 & \cellcolor[HTML]{FCE5CD}0.25 & \cellcolor[HTML]{FFFFFF}0.36 \\
    & CodeLlama(7B) & 0.13 & \cellcolor[HTML]{FCE5CD}0.27 & 0.40 & \cellcolor[HTML]{D9EAD3}0.21 & \cellcolor[HTML]{FFFFFF}0.14 & \cellcolor[HTML]{FFFFFF}0.34 \\
    & DeepSeek-Coder(13B) & 0.20 & \cellcolor[HTML]{FCE5CD}0.23 & 0.43 & \cellcolor[HTML]{D9EAD3}0.24 & \cellcolor[HTML]{FFFFFF}0.11 & \cellcolor[HTML]{FFFFFF}0.34 \\
    & StarCoder(13B) & 0.17 & \cellcolor[HTML]{FCE5CD}0.24 & 0.41 & \cellcolor[HTML]{D9EAD3}0.26 & \cellcolor[HTML]{FFFFFF}0.13 & \cellcolor[HTML]{FFFFFF}0.39 \\
    & CodeLlama(13B) & 0.17 & \cellcolor[HTML]{FCE5CD}0.30 & 0.47 & 0.12 & \cellcolor[HTML]{FCE5CD}0.22 & \cellcolor[HTML]{FFFFFF}0.25 \\
    & DeepSeek-Coder(33B) & 0.15 & \cellcolor[HTML]{FCE5CD}0.29 & 0.44 & \cellcolor[HTML]{D9EAD3}0.24 & \cellcolor[HTML]{FFFFFF}0.21 & 0.45 \\
   \multirow{-8}{*}{} & CodeLlama(34B) & 0.09 & \cellcolor[HTML]{FCE5CD}0.32 & 0.41 & \cellcolor[HTML]{D9EAD3}0.25 & \cellcolor[HTML]{FFFFFF}0.22 & 0.47 \\ \hline
    & GPT-3.5-Turbo & 0.06 & \cellcolor[HTML]{FCE5CD}0.29 & 0.35 & \cellcolor[HTML]{D9EAD3}0.22 & \cellcolor[HTML]{FFFFFF}0.19 & 0.41 \\
   \multirow{-2}{*}{} & GPT-4 & 0.14 & \cellcolor[HTML]{FCE5CD}0.17 & 0.31 & 0.14 & \cellcolor[HTML]{FCE5CD}0.19 & 0.32 \\ \hline
   \multicolumn{1}{l}{} & Average & 0.15 & \cellcolor[HTML]{FCE5CD}0.25 & 0.40 & \cellcolor[HTML]{D9EAD3}0.21 & \cellcolor[HTML]{FFFFFF}0.19 & 0.39 \\ \hline
    \end{tabular}
    \label{tab:rq2}
    \end{table*}

==> src/tf/tab_prompts.tex <==
% \begin{table*}[t]
%     \scriptsize
%         \caption{Different Prompting Methods.\todo{There are still some bugs with left-right alignment}}
%         \setlength{\tabcolsep}{0pt}
%         \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lp{0.75\textwidth}}
%         \hline
%         Prompting Type & Detailed Prompts \\ \hline
%         Directly Input (DI) & {\color[HTML]{0070C0} \{question\}} \\
%         Basic Prompt (BP) & \# Complete the following Python code without any tests or explanation\textbackslash{}n{\color[HTML]{0070C0} \{question\}} \\
%         Quality-aware Prompt (QA) & \# Complete the following Python code by {\color[HTML]{f44336} a concise and efficient} implementation.\textbackslash{}n{\color[HTML]{0070C0} \{question\}} \\
%         CoT Prompt (CoT) & \# Complete the following Python code without any tests or explanation, {\color[HTML]{f44336} let's think step by step}\textbackslash{}n{\color[HTML]{0070C0} \{question\}} \\
%         Quality-aware CoT Prompt (QA+CoT) & \# Complete the following Python code by {\color[HTML]{f44336} a concise and efficient} implementation, {\color[HTML]{f44336} let's think step by step}\textbackslash{}n{\color[HTML]{0070C0} \{question\}} \\ \hline
%         \end{tabular*}
%         \label{tab:prompting}
%     \end{table*}


\begin{table*}[t]
    \scriptsize
        \caption{Different Prompting Methods.\todo{There are still some bugs with left-right alignment}}
        \setlength{\tabcolsep}{0pt}
        \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lp{0.75\textwidth}}
        \hline
        Prompting Type & Detailed Prompts \\ \hline
        Directly Input (DI) & {\color[HTML]{0070C0} \{question\}} \\
        Basic Prompt (BP) & \# Complete the following Python code without any tests or explanation\textbackslash{}n{\color[HTML]{0070C0} \{question\}} \\
        Quality-aware Prompt (QA) & \# Complete the following Python code by {\color[HTML]{f44336} a concise and efficient} implementation.\textbackslash{}n{\color[HTML]{0070C0} \{question\}} \\
        CoT Prompt (CoT) & \# Complete the following Python code without any tests or explanation, {\color[HTML]{f44336} let's think step by step}\textbackslash{}n{\color[HTML]{0070C0} \{question\}} \\
        Quality-aware CoT Prompt (QA+CoT) & \# Complete the following Python code by {\color[HTML]{f44336} a concise and efficient} implementation, {\color[HTML]{f44336} let's think step by step}\textbackslash{}n{\color[HTML]{0070C0} \{question\}} \\ \hline
        \end{tabular*}
        \label{tab:prompting}
    \end{table*}



==> src/trash.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% \begin{table*}[]
%     \caption{Effectiveness measurement results.}
%     \centering
%     \begin{tabular}{|lllllllll|}
%         \hline
%         \multicolumn{1}{|l|}{}                       & \multicolumn{4}{c|}{t = 0.2}                                                                                                             & \multicolumn{4}{c|}{t = 0.8}                                                                    \\
%         \multicolumn{1}{|l|}{\multirow{-2}{*}{LCGM}} & $\text{CR}_{en}$                    & $\text{CR}_{zh}$                    & $\text{CR}_{bi}$  & \multicolumn{1}{l|}{CRD}                     & $\text{CR}_{en}$                    & $\text{CR}_{zh}$                    & $\text{CR}_{bi}$ &  CDR \\ \hline
%         \multicolumn{1}{|l|}{CodeGeeX}               & \cellcolor[HTML]{E2EFDA}0.6  & 0.54                         & 0.54            & \multicolumn{1}{l|}{0.06}                          & 0.62                         & \cellcolor[HTML]{FCE4D6}0.63 & 0.58        & 0.1      & 0.14     \\
%         \multicolumn{1}{|l|}{CodeGen2.5}              & 0.52                         & 0.52                         & 0.46             & \multicolumn{1}{l|}{0.12}                          & 0.46                         & \cellcolor[HTML]{FCE4D6}0.48 & 0.4         & 0.13     & 0.25     \\
%         \multicolumn{1}{|l|}{CodeLlama}              & 0.5                          & \cellcolor[HTML]{FCE4D6}0.54 & 0.46            & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}0.12 }  & \cellcolor[HTML]{E2EFDA}0.52 & 0.5                          & 0.46        & 0.1      & 0.17     \\
%         \multicolumn{1}{|l|}{DeepSeek-Coder}          & \cellcolor[HTML]{E2EFDA}0.63 & 0.58                         & 0.54            & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}0.13 }  & \cellcolor[HTML]{E2EFDA}0.71 & 0.65                         & 0.63        & 0.1      & 0.13     \\
%         \multicolumn{1}{|l|}{StarCoder}              & 0.48                         & \cellcolor[HTML]{FCE4D6}0.52 & 0.44            & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}0.12 } & \cellcolor[HTML]{E2EFDA}0.58 & 0.56                         & 0.52        & 0.1      & 0.16     \\
%         \multicolumn{1}{|l|}{GPT-3.5-Turbo}           & 0.58                         & \cellcolor[HTML]{FCE4D6}0.64 & 0.58        & \textcolor{red}{0.08}     & \multicolumn{1}{l|}{\cellcolor[HTML]{FFFFFF}\textcolor{red}{0.12}} & \cellcolor[HTML]{E2EFDA}0.7  & 0.66                         & 0.67        & \textcolor{red}{0.04}     & \textcolor{red}{0.05}     \\ \hline
%         Average                                      & 0.55                         & 0.56                         & 0.50        & 0.11     & 0.17                                              & 0.60                         & 0.58                         & 0.54        & 0.10     & 0.15     \\ \hline
%         \end{tabular}
%     \label{tab:rq1}

% \end{table*}
